Discovering and Mitigating Visual Biases through Keyword Explanation

Addressing biases in computer vision models is crucial for real-world AI deployments. However, mitigating visual biases is challenging due to their unexplainable nature, often identified indirectly through visualization or sample statistics, which necessitates additional human supervision for interpretation. To tackle this issue, we propose the Bias-to-Text (B2T) framework, which interprets visual biases as keywords. Specifically, we extract common keywords from the captions of mispredicted images to identify potential biases in the model. We then validate these keywords by measuring their similarity to the mispredicted images using a vision-language scoring model. The keyword explanation form of visual bias offers several advantages, such as a clear group naming for bias discovery and a natural extension for debiasing using these group names. Our experiments demonstrate that B2T can identify known biases, such as gender bias in CelebA, background bias in Waterbirds, and distribution shifts in ImageNet-R/C. Additionally, B2T uncovers novel biases in larger datasets, such as Dollar Street and ImageNet. For example, we discovered a contextual bias between "bee" and "flower" in ImageNet. We also highlight various applications of B2T keywords, including debiased training, CLIP prompting, and model comparison.

==> resources/fig_cls-bias.tex <==
\begin{figure*}[t!]
\centering\small
\includegraphics[width=\textwidth]{_cvpr2024/figures/fig_bias-known.pdf}
\includegraphics[width=\textwidth]{_cvpr2024/figures/fig_bias-unknown(a).pdf}
\vspace{-0.16in}
\caption{
\textbf{Discovered biases in image classifiers.}
Visual examples of mispredicted validation samples along with their corresponding bias keywords, captions, actual, and predicted classes. B2T successfully uncovered known biases, such as (a) gender bias in CelebAs blond, (b) background bias in Waterbirds, and (c, d) distribution shifts in ImageNet-R and ImageNet-C. Additionally, B2T discovered novel biases, such as the spurious correlations between (e) \keyword{cave} with the wardrobe class, indicating geographical bias in Dollar Street, and (f) \keyword{flower} with the ant class, indicating scene bias in ImageNet.
}\label{fig:cls-bias}
\vspace{-0.1in}
\end{figure*}

==> resources/tab_cls-bias-label.tex <==
\begin{table}[t]
\caption{
Precision (P), recall (R), and F1-score (F1) of group labels inferred by CLIP zero-shot classifier, using the group names or B2T for prompts.
We \textbf{bold} the best values.
}\label{tab:cls-bias-label}
% \vspace{-0.1in}
\centering\small
\resizebox{\linewidth}{!}{% 
\newcommand{\stdv}[1]{{\scriptsize$\pm$#1}}
\begin{tabular}{l @{\hspace{8pt}} c@{\hspace{4pt}}c@{\hspace{4pt}}c @{\hspace{8pt}} c@{\hspace{4pt}}c@{\hspace{4pt}}c}
\toprule
& \multicolumn{3}{c}{CelebA blond} & \multicolumn{3}{c}{Waterbirds} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
 % & Precision & Recall & F1-score & Precision & Recall & F1-score \\
 & P & R & F1 & P & R & F1 \\
\midrule
% ERM prediction~\citep{liu2021just}  & 0.22 & 0.64 & 0.33  &  0.21 & 0.71 & 0.33 \\
% GEORGE~\citep{sohoni2020no}         & 0.16 & 0.83 & 0.27  &  0.13 & 0.74 & 0.22 \\
% \midrule
% CLIP zero-shot                      & \multirow{2}{*}{\textbf{0.96}} & \multirow{2}{*}{\textbf{0.95}} & \multirow{2}{*}{\textbf{0.96}} & 0.25  & 0.59  & 0.35 \\
% CLIP zero-shot w/ B2T (ours)     &  &  & & \textbf{0.66} & \textbf{0.88} & \textbf{0.76} \\
CLIP w/ group prompt~\citep{zhang2022contrastive}                      & \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & 0.25  & 0.59  & 0.35 \\
CLIP w/ B2T prompt (ours)
% CLIP zero-shot w/ B2T (ours)     
& \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & \textbf{0.66} & \textbf{0.88} & \textbf{0.76} \\
\bottomrule
\end{tabular}}
\vspace{-0.1in}
\end{table}

% \multirow{4}{*}{GS}

==> resources/tab_debias-label.tex <==
\begin{table}[t]
\caption{
Precision (P), recall (R), and F1-score (F1) of group labels inferred by prior methods and CLIP zero-shot classifier, using the group names or B2T for prompts.
We \textbf{bold} the best values. Ours outperforms the prior methods and the base CLIP using group prompts.
}\label{tab:f1score}
% \vspace{-0.1in}
\centering\small
\resizebox{\linewidth}{!}{% 
\newcommand{\stdv}[1]{{\scriptsize$\pm$#1}}
\begin{tabular}{l @{\hspace{8pt}} c@{\hspace{4pt}}c@{\hspace{4pt}}c @{\hspace{8pt}} c@{\hspace{4pt}}c@{\hspace{4pt}}c}
\toprule
& \multicolumn{3}{c}{CelebA blond} & \multicolumn{3}{c}{Waterbirds} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
 % & Precision & Recall & F1-score & Precision & Recall & F1-score \\
 & P & R & F1 & P & R & F1 \\
\midrule
ERM prediction~\citep{liu2021just}  & 0.22 & 0.64 & 0.33  &  0.21 & 0.71 & 0.33 \\
GEORGE~\citep{sohoni2020no}         & 0.16 & 0.83 & 0.27  &  0.13 & 0.74 & 0.22 \\
\midrule
% CLIP zero-shot                      & \multirow{2}{*}{\textbf{0.96}} & \multirow{2}{*}{\textbf{0.95}} & \multirow{2}{*}{\textbf{0.96}} & 0.25  & 0.59  & 0.35 \\
% CLIP zero-shot w/ B2T (ours)     &  &  & & \textbf{0.66} & \textbf{0.88} & \textbf{0.76} \\
CLIP w/ group prompt~\citep{zhang2022contrastive}                      & \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & 0.25  & 0.59  & 0.35 \\
CLIP w/ B2T prompt (ours)
% CLIP zero-shot w/ B2T (ours)     
& \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & \textbf{0.66} & \textbf{0.88} & \textbf{0.76} \\
\bottomrule
\end{tabular}}
\end{table}

% \multirow{4}{*}{GS}

==> sec/7_generative.tex <==
\section{Extension to Generative Models}
\label{sec:generative}
We extend B2T framework to text-to-image generative models. Here, we define biases as unintended attributes that are not explicitly specified through prompts.

\subsection{B2T for text-to-image generative models}
Text-to-image (T2I) generative models produce an image $x \in \mathcal{X}$ from a given text description $y \in \mathcal{Y}$. Our goal is to identify a biased attribute $a \in \mathcal{A}$ that is spuriously correlated with the input prompts, i.e., the generated images $x$ contain the biased attribute $a$ even though it is not explicitly described in $y$. For example, a generative model may produce only female images when conditioned on blond, suggesting that the attribute \keyword{woman} is spuriously correlated with the prompt \keyword{blond.}

To identify the biased attribute $a$, we extract common keywords from the captions of the \textit{generated} images, rather than the mispredicted ones for classifiers. The keywords that appear in the generated images can be either the intended text $y$ or unintended bias $a$, and the user can infer the candidate set of biased keywords. In the case of the generative model conditioned on the prompt \keyword{blond,} the keywords \keyword{woman} (as well as \keyword{blond}) will frequently appear.


However, this simple approach has a potential issue in that the captioning model may exhibit bias, as we discussed for the classifiers. It may misleadingly produce certain words frequently, even though they are not the majority keywords in the generated images. Therefore, we additionally define a metric that verifies whether the generated images indeed reflect the unintended bias keywords. This metric requires that the underlying generative model is a T2I diffusion model~\citep{sohl2015deep,ho2020denoising}. We use the Stable Diffusion (SD)~\citep{rombach2022highresolution} in our experiments and refer to our metric as the SD score\footnote{
%
Details of the SD score are illustrated in Appendix~\ref{appx:bias-gen}
%
}.

\input{resources/fig_gen-bias}
\subsection{Bias discovery for generative models} 
% Detailed discussions can be found in Appendix~\ref{appx:bias-gen}, and the complete list of keywords is included in Appendix~\ref{appx:more-table-gen}.

We apply B2T on Stable Diffusion~\citep{rombach2022highresolution} using the prompts from~\citep{luccioni2023stable, friedrich2023fair}, which result in the unfair generation of images. B2T recovers known biases, such as spurious correlations between occupations and gender or race. For instance, as shown in Figure~\ref{fig:gen-bias}, we find that Stable Diffusion associates nurses with \keyword{women} and construction workers with \keyword{men,} indicating gender bias, and maids with \keyword{Asians,} indicating racial bias. Moreover, B2T uncovers unknown biases from the same prompts, such as the association of nurses with \keyword{stethoscope,} construction workers with \keyword{hat,} and Native Americans with \keyword{feathers,} suggesting that the model exhibits stereotypes based on the appearance of certain occupations and ethnicities.

% \subsection{Debiasing generative models with B2T}
% \input{resources/fig_gen-debias}

% We use the bias keywords to debias a T2I diffusion model, Stable Diffusion~\citep{rombach2022highresolution}. To achieve this, we apply the Fair Diffusion~\citep{friedrich2023fair} algorithm, which adjusts the diffusion score that used to update images during generation, in order to regulate the effects of the specified keywords.

% Figure~\ref{fig:gen-debias} demonstrates that Fair Diffusion, utilizing the bias keywords discovered by B2T, effectively eliminates the biases mentioned earlier. Our approach balances the unfair generation of images. We believe that B2T can facilitate the desirable use of fair T2I generative models.

==> sec/7_limitation.tex <==
\section{Limitations}
\label{sec:limitation}


% \textbf{Limitations.}
% There is a potential risk that the pre-trained models themselves may exhibit bias~\citep{agarwal2021evaluating}. Thus, users should not fully rely on the extracted captions, and the involvement of human juries remains crucial. For example, CLIP is primarily trained on natural images and may be less effective in specialized domains such as medical or satellite imaging. Thus, training a specialized captioning model is necessary for applying B2T to these domains.

% Despite the fact that the concept of B2T is generally applicable to arbitrary bias keywords, it may fail to capture some words as captions do not explain every aspects of the images. However, we demonstrate that current captioning models can well capture the inherent biases in various scenarios, and we believe that the rapid advance in pre-trained models such as GPT-4~\citep{openai2023gpt} will eventually resolve this issue.


% \textbf{Ethical concerns.}
% Bias and fairness research inherently carries the potential for negative social impacts. It is important to emphasize that the goal of B2T is not to \textit{fully automate} the process of finding biases, but rather to \textit{assist} humans in making decisions based on suggested bias keywords. The ultimate judgment should be entrusted to the users.

% In our study, we utilize sensitive examples, including gender and geographic biases. It is crucial to note that our intention is to raise awareness and mitigate potential risks in real-world datasets publicly accessible through platforms like Kaggle or Dollar Street websites.


% \textbf{Future works.} We discuss various applications of B2T, including discovering unknown biases in datasets, analyzing behaviors of classifiers, and debiasing zero-shot and full-shot classifiers. Applying B2T to more challenging real-world problems would be an exciting and impactful future direction. Also, one can extend B2T for creating a fairness or bias benchmark using the B2T bias keywords or designing a robust classifier by comparing models with B2T.
